ControlVAE: Tuning, Analytical Properties, and Performance Analysis

This paper reviews the novel concept of controllable variational autoencoder (ControlVAE), discusses its parameter tuning to meet application needs, derives its key analytic properties, and offers useful extensions and applications. ControlVAE is a new variational autoencoder (VAE) framework that combines the automatic control theory with the basic VAE to stabilize the KL-divergence of VAE models to a specified value. It leverages a non-linear PI controller, a variant of the proportional-integral-derivative (PID) control, to dynamically tune the weight of the KL-divergence term in the evidence lower bound (ELBO) using the output KL-divergence as feedback. This allows us to precisely control the KL-divergence to a desired value (set point), which is effective in avoiding posterior collapse and learning disentangled representations. In order to improve the ELBO over the regular VAE, we provide simplified theoretical analysis to inform setting the set point of KL-divergence for ControlVAE. We observe that compared to other methods that seek to balance the two terms in VAE's objective, ControlVAE leads to better learning dynamics. In particular, it can achieve a good trade-off between reconstruction quality and KL-divergence. We evaluate the proposed method on three tasks: image generation, language modeling and disentangled representation learning. The results show that ControlVAE can achieve much better reconstruction quality than the other methods for comparable disentanglement. On the language modeling task, ControlVAE can avoid posterior collapse (KL vanishing) and improve the diversity of generated text. Moreover, our method can change the optimization trajectory, improving the ELBO and the reconstruction quality for image generation.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> back.model.tex <==
\section{The ControlVAE Algorithm}
\label{sec:model}
During model training, we sample the output KL-divergence, which we denote by $\hat{v}_{kl}(t)$, at training step $t$. The sampled KL-divergence is then compared to the set point, ${v}_{kl}$, and the difference, $e(t) = {v}_{kl} - \hat{v}_{kl}(t)$, then used as the feedback to a controller to calculate the hyperparameter $\beta(t)$. ControlVAE can be expressed by the following variational lower bound:
\begin{equation}\label{eq:controlVAE-object}
\mathcal{L} = \mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})} [\log p_\theta(\mathbf{x|z})] - \beta(t) KL(q_\phi(\mathbf{z}|\mathbf{x})||p(\mathbf{z})).
\end{equation}


%%%%--design PI control algorithm
When KL-divergence drops below the set point, the controller counteracts this change by reducing the hyperparameter $\beta(t)$ (to reduce penalty for KL-divergence in the objective function~\eqref{eq:controlVAE-object}). The reduced weight, $\beta(t)$, allows KL-divergence to grow, thus approaching the set point again. Conversely, when KL-divergence grows above the set point, the controller increases $\beta(t)$ (up to a certain value), thereby increasing the penalty for KL-divergence and forcing it to decrease. This effect is achieved by computing $\beta(t)$ using Equation~(\ref{eq:vae-lang}), below, which is an instance of nonlinear PI control: \begin{equation}\label{eq:vae-lang}
\vspace{-0.02in}
\beta(t) = \frac{K_p}{1+\exp(e(t))} - K_i \sum_{j=0}^t e(j) + \beta_{min},
\end{equation}
where $K_p$ and $K_i$ are the constants. The first term (on the right hand side) ranges between $0$ and $K_p$ thanks to the exponential function $exp(.)$. Note that when error is large and positive (KL-diverge is below set point), the first term approaches 0, leading to a lower $\beta(t)$ that encourages KL-divergence to grow. Conversely, when error is large and negative (KL-divergence above set point), the first term approaches its maximum (which is $K_p$), leading to a higher $\beta(t)$ that encourages KL-divergence to shrink.

The second term of the controller sums (integrates) past errors with a sampling period $T$ (one training step in this paper). This creates a progressively stronger correction (until the sign of the error changes). The negative sign ensures that while errors remain positive (i.e., when KL-divergence is below set point), this term continues to decrease, whereas while errors remain negative (i.e., when KL-divergence is above set point), this term continues to increase. In both cases, the change forces $\beta(t)$ in a direction that helps KL-divergence approach the set point. In particular, note that when the error becomes zero, the second term (and thus the entire right hand side) stops changing, allowing controller output, $\beta(t)$, to stay at the same value that hopefully caused the zero error in the first place. This allows the controller to ``lock in" the value of $\beta(t)$ that meets the KL-divergence set point.
Finally, $\beta_{min}$ is an application-specific constant. It effectively shifts the range within which $\beta(t)$ is allowed to vary. This PI controller is illustrated in Fig.~\ref{fig:pid}.

%%figure%%
\begin{figure}[!t]
\begin{center}
\centerline{\includegraphics[width=0.99\columnwidth]{figures/pid.pdf}}
\caption{The block diagram of PI controller. It uses the output KL-divergence at training step $t$ as the feedback to the PI algorithm to compute $\beta(t)$.}
\label{fig:pid}
\end{center}
\end{figure}


\subsection{The Controllable FactorVAE Algorithm}
\label{sec:control-factorVAE}
For disentangled representation learning, the total correlation (TC) term of FactorVAE may collapse to 0, leading to bad disentanglement. To deal with this issue, we propose a novel controllable FactorVAE, Control-FactorVAE, to stabilize the TC to a small value based on the actual value of TC during model training. Similar to ControlVAE, the objective function of Control-FactorVAE is expressed as
\begin{equation}\label{eq:control-factor}
\begin{split}
\mathcal{L}_{f} & =  \mathbb{E}_{q_\phi(\mathbf{z|x)}} [\log p_\theta(\mathbf{x|z})] - KL (q_\phi(\mathbf{z|x})||p(\mathbf{z})) \\
&- \beta(t)  KL (q(\mathbf{z})||\bar{q}(\mathbf{z})),
\end{split}
\end{equation}
where $\beta(t)$ is the output of the above designed PI controller using the output TC as feedback.

%%%subsection PID
\subsection{PI Parameter Tuning for ControlVAE}
\label{sec:pi_tuning}
One challenge of applying the PI control algorithm lies how to tune its parameters, $K_p$ and $K_i$ effectively. While optimal tuning of nonlinear controllers is non-trivial, in this paper we follow a very simple rule: tune these constants to ensure that reactions to errors are sufficiently smooth to allow gradual convergence.
Let us first consider the coefficient $K_p$. Observe that the maximum (positive) error occurs when actual KL-divergence is close to zero. In this case, if $v_{kl}$ is the set point on KL-divergence, then the error, $e(t)$, is approximated by $e(t) \approx v_{kl} - 0 = v_{kl}$. When KL-divergence is too small, the VAE does not learn useful information from input data~\cite{liu2019cyclical}. We need to assign $\beta(t)$ a very small non-negative value, so that KL-divergence is encouraged to grow (when the resulting objective function is optimized). In other words, temporarily ignoring other terms in Equation~\eqref{eq:vae-lang}, the contribution of the first term alone should be sufficiently small:
\begin{equation}\label{eq:Kp}
\frac{K_p}{1+\exp( v_{kl} )} \leq \epsilon,
\end{equation}
where $\epsilon$ is a small constant (e.g., $10^{-3}$ in our implementation). The above~\eqref{eq:Kp} can also be rewritten as $K_p \leq (1+\exp(v_{kl}))\epsilon$. Empirically, we find that $K_p=0.01$ leads to good performance and satisfies the above constraint.


Conversely, when the actual KL-divergence is much larger than the desired value $v_{kl}$, the error $e(t)$ becomes a large negative value. As a result, the first term in~\eqref{eq:vae-lang} becomes close to a constant, $K_p$. If the resulting larger value of $\beta(t)$ is not enough to cause KL-divergence to shrink, one needs to gradually continue to increase $\beta(t)$. This is the job of second term. 
The negative sign in front of that term ensures that when negative errors continue to accumulate, the positive output $\beta(t)$ continues to increase. Since it takes lots of steps to train deep VAE models,
the increase per step should be very small, favoring smaller values of $K_i$. 
Empirically we found that a value $K_i$ between $10^{-3}$ and $10^{-4}$ stabilizes the training. Note that, $K_i$ should not be too small either, because it would then unnecessarily slow down the convergence.



%%%%%bound of set point %%%
\subsection{Set Point Guidelines for ControlVAE}
\label{sec:bound}
The choice of desired value of KL-divergence (set point) is largely application specific. In general, when $ \beta_{min} \leq \beta(t) \leq \beta_{max}$, the upper bound of expected KL-divergence is the value of KL-divergence as ControlVAE converges when $\beta(t) = \beta_{min}$, denoted by $V_{max}$. Similarly, its lower bound, $V_{min}$, can be defined as the KL-divergence produced by ControlVAE when $\beta(t) = \beta_{max}$. For feedback control to be most effective (i.e., not run against the above limits), the KL-divergence set point should vary in the range of $[V_{min}, V_{max}]$. Since ControlVAE is an end-to-end learning model, users can customize the desired value of KL-divergence (using KL-divergence of the original VAE as a reference) to meet their demand with respect to different applications. For instance, if some users prefer to improve the diversity of text generation and image generation, they can slightly increase the KL-divergence produced by the original VAE. Otherwise they can reduce the KL-divergence if they want to improve the generation accuracy.

In this paper, we provide a simplified theoretical analysis about how to choose the set point if our goal is to improve the ELBO or the reconstruction accuracy over the basic VAE. Let $d$ ($d>0$) denote the optimal range of KL-divergence between ControlVAE and the basic VAE, and $KL_{vae}$ denote the value of KL-divergence as the basic VAE converges. Then the KL-divergence of ControlVAE can be denoted by
\begin{equation}
KL_{cvae} = KL_{vae} + d.
\end{equation}
\noindent
Therefore, the ELBO of the ControlVAE can be written as
\begin{equation}
\mathcal{L}_{cvae} =  \mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})} [\log p_\theta(\mathbf{x|z})] - (KL_{vae} + d)
\end{equation}

In order to achieve a higher ELBO for ControlVAE, we want
\begin{equation}\label{eq:elbo_compare}
\begin{split}
 & \mathcal{L}_{cvae}  - \mathcal{L}_{vae}  =  \\
 &\mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})} [\log p_\theta(\mathbf{x|z})] - \mathbb{E}_{q_{\phi'}(\mathbf{z_0|x)}} [\log p_{\theta'}(\mathbf{x|z}_0)] -d \geq 0,
 \end{split}
\end{equation}
where $\mathbf{z}$ and $\mathbf{z}_0$ denote the latent variable of ControlVAE and the original VAE, respectively. Since the KL term mainly affects the encoder parameters, to simplify analysis, we may assume that $\theta \approx \theta'$. 

In order to obtain the range $d$, our next step is to bound the difference of reconstruction accuracy between ControlVAE and the basic VAE, $\mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})} [\log p_\theta(\mathbf{x|z})] - \mathbb{E}_{q_\phi(\mathbf{z_0|x)}} [\log p_\theta(\mathbf{x|z}_0)]$. Assuming the decoder to be Lipschitz continuous~\cite{virmaux2018lipschitz}, we have the following theorem.
\begin{theorem}\label{the:z_eq}
Given the KL-divergence, $KL_{vae}$, of the original VAE as it converges, we have
\begin{equation}\label{eq:z_range}\small
\mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})} [\log p_\theta(\mathbf{x|z})] - \mathbb{E}_{q_\phi(\mathbf{z_0|x)}} [\log p_\theta(\mathbf{x|z}_0)]  \leq   \sqrt{ 4(2KL_{vae}+d)}.
\end{equation}
\end{theorem}
\noindent
\textit{Proof:} please see it in Appendix~\ref{app:theorem1}.

\noindent
Based on the above Theorem~\ref{the:z_eq} and Eq.~\eqref{eq:elbo_compare}, we have
\begin{equation}\label{eq:lipt_eta}
0 \leq d \leq \sqrt{ 4(2KL_{vae}+d)},
\end{equation}
From the above equation, we can derive the range $d$:
\begin{equation}
0  \leq d \leq 2 + 2\sqrt{2KL_{vae} +1 }.
\end{equation}
Therefore, if we choose $d$ in the above range, we can improve the ELBO of ControlVAE.



%%%%%algorithm%%%
\subsection{Summary of the PI Control Algorithm}
We summarize the proposed PI control algorithm in Algorithm~\ref{alg:pid}. Our PI algorithm updates the hyperparameter, $\beta(t)$, with the feedback from sampled KL-divergence at training step $t$. Line $6$ computes the error between the desired KL-divergence, $v_{kl}(t)$, and the sampled $\hat{v}_{kl}(t)$. Line $7$ to $9$ calculate the P term and I term for the PI algorithm, respectively. Note that, Line 10 and 11 is a popular constraint in PID/PI design, called anti-windup~\cite{azar2015design,peng1996anti}. It effectively disables the integral term of the controller when controller output gets out of range, not to exacerbate the out-of-range deviation. Line $13$ is the calculated hyperparameter $\beta(t)$ by PI algorithm in~\eqref{eq:vae-lang}. Finally, Line $14$ to $19$ aim to limit $\beta(t)$ to a certain range, $[\beta_{min},\beta_{max}]$.

%%%--PID algorithm----
% \vspace{-0.1in}
\begin{algorithm}[!tb]
   \caption{PI algorithm.}
   \label{alg:pid}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} desired KL $v_{kl}$, coefficients $K_p$, $K_i$, max/min value $\beta_{max}$, $\beta_{min}$, iterations $N$
   \STATE {\bfseries Output:} hyperparameter $\beta(t)$ at training step $t$
%   %\REPEAT
   \STATE {\bfseries Initialization}: $I(0)=0$, $\beta(0)=0$
   \FOR{$t=1$ {\bfseries to} $N$}
   \STATE Sample KL-divergence, $\hat{v}_{kl}(t)$
   \STATE $e(t) \leftarrow v_{kl}-\hat{v}_{kl}(t)$
   \STATE $P(t) \leftarrow \frac{K_p}{1+\exp(e(t))}$
   \IF{ $ \beta_{min} \leq \beta(t-1) \leq \beta_{max}$ }
   		\STATE $I(t) \leftarrow I(t-1) - K_i e(t)$
   \ELSE
   \STATE $I(t) = I(t-1)$ \quad // Anti-windup
	 \ENDIF
   \STATE $\beta(t)=P(t)+I(t) + \beta_{min}$
   \IF{$\beta(t)> \beta_{max}$}
   \STATE $\beta(t)= \beta_{max}$
 	\ENDIF
   \IF{$\beta(t)< \beta_{min}$}
   \STATE $\beta(t)= \beta_{min}$
   \ENDIF
   \STATE \textbf{Return} $\beta(t)$
 \ENDFOR
\end{algorithmic}
\end{algorithm}

% {\color{blue}
%%% steady state error
% \subsection{Stability Analysis for ControlVAE}
% We try to theoretically analyze the stability of the proposed ControlVAE. Our first step is to build its nonlinear state space model. In this paper, the state variable at training step $t$ is defined as
% \begin{equation}\label{eq:state_x}
% x(t)= \beta(t)
% \end{equation}
% According to the diagram in Fig.~\ref{fig:pid}, we have
% \begin{equation}\label{eq:state_beta}
% \left\{
% \begin{aligned}
% & \beta(t) = K_p\sigma(e(t))-K_i\sum_{j=1}^{t} e(j) + \beta_{min} \\
% & KL(t) = g(\beta(t)) \\
% & e(t+1) = v_{kl} - g(\beta(t)), \\
% \end{aligned}
% \right.
% \end{equation}
% \noindent
% where $\sigma(e(t))= \frac{1}{(1+exp(e(t))}$ and $g(.)$ denotes the transfer function between $\beta(t)$ and the output KL-divergence $KL(t)$. Fig.~\ref{fig:fitting} shows the output $KL(t)$ varies with the increase of $\beta(t)$ in an open-loop control system (i.e., $\beta$-VAE in Eq.~\eqref{eq:beta-vae}) via doing experiments on CIFAR10 data set. We can observe that the actual $KL(t)$ and $\beta(t)$ have a negative correlation.

% \begin{figure}[!t]
% \begin{center}
% \centerline{\includegraphics[width=0.93\columnwidth]{figures/Fitting.pdf}}
% \caption{The relationship between the actual output $KL(t)$ and $\beta(t)$.}
% \label{fig:fitting}
% \end{center}
% \end{figure}


% Based on Eqs.~\eqref{eq:state_x}\eqref{eq:state_beta}, the state variable $x(t)$ and $x(t+1)$ can be rewritten as
% \begin{subequations}\small
% \begin{align}
% & x(t+1) = \beta(t+1) = K_p\sigma(e(t+1))-K_i\sum_{j=1}^{t+1} e(j) + \beta_{min}  \label{eq:x_n1}\\
% & x(t) = \beta(t) = K_p\sigma(e(t))-K_i\sum_{j=1}^{t} e(j) \label{eq:x_n} + \beta_{min}
% \end{align}
% \end{subequations}
% Subtracting Eq.~\eqref{eq:x_n} from \eqref{eq:x_n1}, we have

% \begin{equation}\label{eq:x_sub}\small
% \begin{split}
% x(t+1)-x(t) &= K_p [e(t+1)-e(t)] - K_i e(t+1) \\
% &=K_p(\sigma[v_{kl}-g(x(t))]-\sigma[v_{kl}-g(x(t-1))]) \\
% & - K_i[v_{kl}-g(x(t))]
% \end{split}
% \end{equation}

% \noindent
% The above Eq.~\eqref{eq:x_sub} is a second-order discrete control system. Let state variables $x_1(t)=x(t)$ and $x_2(t)=x_1(t-1)=x(t-1)$, then the above state space can be expressed by $x_1(t)$ and $x_2(t)$ below.
% \begin{equation}\label{eq:2nd_order}
% \left\{
% \begin{aligned}
% x_1(t+1) & = f_1(x_1(t), x_2(t)) \\
% & = x_1(t) - K_i[v_{kl}-g(x_1(t))] + \\
% & K_p(\sigma[v_{kl}-g(x_1(t))]-\sigma[v_{kl}-g(x_2(t))]) \\
% x_2(t+1)& =f_2(x_1(t), x_2(t))=x_1(t)\\
% \end{aligned}
% \right.
% \end{equation}
% In order to analyze the stability of the above non-linear discrete system, one commonly used method is to adopt "linearization" at an equilibrium point~\cite{hughes2015applications}. In this paper, we use the following equilibrium point:
% \begin{equation}
% (x_1^*, x_2^*)=(g^{-1}(v_{kl}), g^{-1}(v_{kl})),
% \end{equation}
% where $g^{-1}(.)$ denotes the inverse function and $x_1^* = x_2^*$.

% For the above Eq.~\eqref{eq:2nd_order}, we use the first order Taylor expself.drop_out1 = nn.Dropout(p)self.drop_out1 = nn.Dropout(p)ansion to get
% \begin{equation}
% X(t+1)=AX(t),
% \end{equation}
% where 
% \begin{equation}
% X(t)=[x_1(t)-x_1^*, x_2(t)-x_2^*]^T,
% \end{equation}
% and $A$ is the Jacobian matrix at equilibrium point, denoted by $x^*$, due to $x_1^* = x_2^*$,
% \begin{equation}
% \begin{split}
% A & = 
% \begin{bmatrix}
% \frac{\partial f_1}{\partial x_1} & \frac{\partial f_1}{\partial x_2}\\
% \frac{\partial f_2}{\partial x_1} & \frac{\partial f_2}{\partial x_2}\\
% \end{bmatrix}_{|x_1=x^*,x_2=x^*} \\
% &=
% \begin{bmatrix}
% 1 + (\frac{1}{4}K_p+K_i)g'(x^*) & -\frac{1}{4}K_pg'(x^*) \\
% 1 & 0 \\
% \end{bmatrix}
% \end{split}
% \end{equation}

% According to Theorem 2 in the literature~\cite{kaczorek2015positivity}, the positive discrete linear system is asymptotically stable if and only all coefficients $a_i$ of the following polynomial are positive:
% \begin{equation}
% det\left[I_n(z+1)-A \right] = z^n + a_{n-1}z^{n-1} + \cdots + a_1z + a_0
% \end{equation}
% In other words, we need to meet two conditions: i) coefficients are positive; ii) linear system is positive.
% We first check the coefficients of the polynomial below
% \begin{equation}\small
% \begin{split}
% & \mathrm{det}\left[I_2(z+1)-A \right] = \left| 
% \begin{array}{cc}
% z-(\frac{1}{4}K_p+K_i)g'(x^*) & \frac{1}{4}K_pg'(x^*) \\
% -1 & z+1
% \end{array}
% \right| \\
% & = z^2 + \left[1-(\frac{1}{4}K_p+K_i)g'(x^*)\right]z - K_i g'(x^*)
% \end{split}
% \end{equation}
% As we know from Fig.~\ref{fig:fitting}, $g'(x^*)<0$ because it is a decreasing function, and $K_p$ and $K_i$ are set to $0.01$ and $10^{-3}$ ($10^{-4}$) respectively in Section~\ref{sec:pi_tuning}, so it is easy to derive that the coefficients are positive. Namely,
% \begin{equation}
% \left\{
% \begin{aligned}
% & 1 - (\frac{1}{4}K_p+K_i)g'(x^*) > 0 \\
% & - K_i g'(x^*) > 0 
% \end{aligned}
% \right.
% \end{equation}

% \noindent
% To meet the second requirement, our next step is to figure out the conditions to guarantee discrete linear system is positive. Based on the definition in~\cite{farina2011positive}, the control system is positive when all the entries in $A$ is nonnegative. Accordingly, we have the following conditions:
% \begin{subequations}
% \begin{align}
% & 1 + (\frac{1}{4}K_p+K_i)g'(x^*) > 0 \label{eq:cond1}\\
% & -\frac{1}{4}K_pg'(x^*) > 0 \label{eq:cond2}
% \end{align}
% \end{subequations}

% Since Eq.~\eqref{eq:cond2} always meets the requirement, we only need to guarantee Eq.~\eqref{eq:cond1} meets the above condition as well. Before that, we first figure out the mapping function $g(\beta(t))$ between $\beta(t)$ and $KL(t)$ in Fig.~\ref{fig:fitting}. We can observe from the (red) data points that a negative exponential function can be approximately obtained by curve fitting, which is given by
% \begin{equation}
% g(\beta(t)) = K\exp(-\lambda \beta(t)) .
% \end{equation}
% Then its derivative is given by
% \begin{equation}
% g'(\beta(t)) = -K \lambda\exp(-\lambda \beta(t)).
% \end{equation}
% Take image generation on CIFAR10 as example. We can fit the curve in Fig.~\ref{fig:fitting} with the following negative exponential function (note that $x(t)=\beta(t)$):
% \begin{equation}
% g(x(t)) = 171.2 \exp(-0.29x(t)),
% \end{equation}
% and the corresponding derivative can be written as
% \begin{equation}\label{eq:g_cifar10}
% g'(x(t)) = -49.65 \exp(-0.29x(t)) \geq -49.65.
% \end{equation}
% Referring to Eq.~\eqref{eq:g_cifar10}, $K_p=0.01$ and $K_i=0.001$, we can know that the condition of Eq.~\eqref{eq:cond1} is always satisfied.

% Similarly, for disentangled representation learning, we can fit the curve $g(x(t))$ using the following exponential function:
% \begin{equation}
% g(x(t)) = 25.69 \exp(-0.072x(t)),
% \end{equation}
% Likewise, we can prove that the condition of Eq.~\eqref{eq:cond1} is satisfied.
% Therefore, based on the above analysis, we prove the stability of the designed ControlVAE system.
% }


% We analyze the steady-state error to demonstrate the designed PI controller can stabilize the KL-divergence to the set point. Since ControlVAE is a discrete control system, Z-transform is used in this paper. Fig.~\ref{fig:z_pid} illustrates the block diagram of closed-loop PI control system using Z-transform.

% \begin{figure}[!t]
% \begin{center}
% \centerline{\includegraphics[width=0.99\columnwidth]{figures/Z_transform.pdf}}
% \caption{The block diagram of PI control system using Z-transform.}
% \label{fig:z_pid}
% \end{center}
% \end{figure}

% According to Fig.~\ref{fig:z_pid}, the error, $E(z)$, can be formulated as
% \begin{equation}\label{eq:Ez}
% E(z) = V(z) - KL(z).
% \end{equation}
% The output KL-divergence can be written as
% \begin{equation}\label{eq:KL_z}
% \begin{split}
% KL(z) & = \beta(z) L(z) \\
%  & = \left[K_p f(E(z)) - \frac{ K_i z}{z-1}E(z) \right] L(z),
% \end{split}
% \end{equation}

% \noindent
% where $f(E(z))$ in P term is a sigmoid function, which is bounded in the range $[0,1]$. Hence, we can approximate the first term as $c K_p$, where $c \in [0,1]$. Then the above Eq.~\eqref{eq:KL_z} is approximated as
% \begin{equation}\label{eq:KL_z2}
% KL(z) = \left[cK_p  - \frac{K_i z}{z-1}E(z) \right] L(z).
% \end{equation}

% \noindent
% Based on Eq.~\eqref{eq:Ez} and \eqref{eq:KL_z2}, we can obtain the error
% \begin{equation}\label{eq:error_z}
% E(z) = \frac{V(z)- c K_p L(z)}{1+G(z)},
% \end{equation}
% where
% \begin{equation}\label{eq:Gz}
% G(z) =  -\frac{K_i z}{z-1} L(z).
% \end{equation}

% \noindent
% Using final-value theorem (FVT) for z-transforms, we have
% \begin{equation}\label{eq:e_fvt}
% \begin{split}
% & \lim_{t \to \infty}  e(t)  = \lim_{z \to 1} (1-z^{-1}) E(z) \\
% & = \lim_{z \to 1} (1-z^{-1}) \frac{V(z)- cK_p L(z)}{1+G(z)} \\
% & = \lim_{z \to 1} (1-z^{-1})  \left[ \frac{V(z)}{1+G(z)} - \frac{c K_p L(z)}{1+G(z)} \right].
% \end{split}
% \end{equation}
% Next, we analyze the steady-state error of each term in the above Eq.~\eqref{eq:e_fvt}. In this paper, the input $V(z)$ is a step input, given by
% \begin{equation}
% V(z)=\frac{1}{1-z^{-1}}v_{kl},
% \end{equation}
% where $v_{kl}$ is the set point of KL-divergence for ControlVAE.

% \noindent
% Then the first term in Eq.~\eqref{eq:e_fvt} can be expressed by
% \begin{equation}\label{eq:first_term}
%  \lim_{z \to 1} (1-z^{-1})  \frac{V(z)}{1+G(z)}  =  \frac{v_{kl}}{1+\lim_{z \to 1}G(z)}.
% \end{equation}
% Our next step is to compute the value of $\lim_{z \to 1}G(z)$ in Eq.~\eqref{eq:Gz}. Consider $L(z)$ is related to the VAE objective and $\beta(t)>0$, it is easy to justify that $\lim_{z \to 1} L(z) \neq 0$ when the KL-divergence is not zero. Hence, we can have
% \begin{equation}
% \lim_{z \to 1}G(z)= \infty.
% \end{equation}
% Thus, the first term in Eq.~\eqref{eq:first_term} becomes $0$.

% \noindent
% For the second term, since $\lim_{z \to 1}G(z)= \infty$, we can approximate it as
% \begin{equation}
% \lim_{z \to 1} (1-z^{-1})  \frac{c K_p L(z)}{G(z)} = - \lim_{z \to 1}  (1-z^{-1})^2 \frac{cK_p}{K_i} = 0
% \end{equation}
% Based on the above analysis, we can conclude that the steady-state error of ControlVAE is zero, which means it can stabilize the KL-divergence to a desired value.
% }

 %%%%connection
\subsection{Connection to Other Models}\label{sec:connect}
We are going to illustrate the connection between ControlVAE and some other existing VAE models.
\subsubsection{Connection to Lagrange Multiplier}
The goal of ControlVAE is to dynamically tune the weight on KL term to stabilize the KL-divergence to a desired value, $v_{kl}$. Inspired by literature~\cite{rezende2018taming}, we can also formulate it as a constrained optimization problem
\begin{equation}
\begin{aligned}
\min_{\phi, \theta} \quad &  \mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})} [\log p_\theta(\mathbf{x|z})]\\
\textrm{s.t.} \quad & KL(q_\phi(\mathbf{z}|\mathbf{x})||p(\mathbf{z})) - v_{kl} = 0\\
\end{aligned}
\end{equation}
The Lagrangian of this optimization problem is
\begin{equation}
\mathcal{L}_m = \mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})} [\log p_\theta(\mathbf{x|z})] - \lambda (KL(q_\phi(\mathbf{z}|\mathbf{x})||p(\mathbf{z})) - v_{kl}),
\end{equation}
where $\lambda$ is the Lagrange multiplier.

\noindent
The above problem could be solved by classic gradient descent-ascent. In particular, the gradient with respect to the Lagrange multiplier $\lambda$ at the $i$-th iteration is given by
\begin{equation}
d\lambda {(i)} = \frac{\partial \mathcal{L}_m }{\partial \lambda} = v_{kl} - KL(q_\phi(\mathbf{z}|\mathbf{x})||p(\mathbf{z})) = e(i),
\end{equation}
where $e(i)$ is the error between the desired KL-divergence and the actual one, as defined in Section~\ref{sec:model}.
\noindent
At training step $i$, we can update $\lambda$ as follows:
\begin{equation}
\begin{split}
\lambda {(i)} & = \lambda {(i-1)} - \alpha d\lambda {(i)} \\
& = \lambda {(i-1)} - \alpha e(i)
\end{split}
\end{equation}
where $\alpha$ is the learning rate.

\noindent
After training the above model with $t$ iterations, the hyperparameter, $\lambda$, can be expressed by
\begin{equation}\label{eq:lambda}
\lambda {(t)} = \lambda {(0)} -\alpha \sum_{i=0}^t  e(i).
\end{equation}
When $\lambda$ is initialized with 0, the above Eq.~\eqref{eq:lambda} becomes
\begin{equation}
\lambda {(t)} = -\alpha \sum_{i=0}^t  e(i).
\end{equation}
\noindent
It can be observed from the above formula that $\lambda(t)$ is the same as I term of the designed PI algorithm in Eq.\eqref{eq:vae-lang} when $\alpha=K_i$. Thus, the optimization problem using Lagrange multiplier can be seen as a special case of ControlVAE. We also conduct experiments to compare the performance of ControlVAE with Lagrange multiplier method in Section~\ref{sec:evaluate}.

\subsubsection{Connection to VAE and $\beta$-VAE}
For the basic VAE, we have $\beta = 1$ on the KL term in the VAE objective. After model training, the KL-divergence of the basic VAE converges to a value, $KL_{vae}$.  When we set the target KL-divergence, $v_{kl}$, to $KL_{vae}$, ControlVAE becomes the basic VAE as the weight $\beta(t)$ converges to $1$ at the end of model training. For the $\beta$-VAE, it assigns a large and fixed weight to the KL term. As long as we fix the output of PI controller as a large value, ControlVAE then becomes $\beta$-VAE.

%%%Application%%%%
\subsection{Applications of ControlVAE}
As a preliminary demonstration of the general applicability of the above approach and as an illustration of its customizability, we apply ControlVAE to three different applications stated below.
\begin{itemize}
%%%% disentangling%%%%%%
\item \textbf{Disentangling}: We then apply the ControlVAE model to achieve a better trade-off between reconstruction quality and disentangling. As mentioned in Section~\ref{sec:beta-vae}, $\beta$-VAE ($\beta>1$) assigns a large hyperparameter to the objective function to control the KL-divergence (information bottleneck), which, however, leads to a large reconstruction error. To mitigate this issue, we adopt ControlVAE to automatically adjust the hyperparameter $\beta(t)$ based on the output KL-divergence during model training. Using the similar methodology in~\cite{burgess2018understanding}, we train a single model by gradually increasing KL-divergence from $0.5$ to a desired value $C$ with a step function $\alpha$ for every $K$ training steps. Since $\beta(t)>1$, we set $\beta_{min}$ to $1$ for the PI algorithm in~\eqref{eq:vae-lang}. Following the PI tuning method above, the coefficients $K_p$ and $K_i$ are set to $0.01$ and $0.001$, respectively.

%%%%%%%%image generation
\item \textbf{Image generation}: In this paper, we try to leverage ControlVAE to manipulate (slightly increase) the value of KL-divergence to improve the ELBO and reconstruction quality over the basic VAE for image generation. Different from the original VAE ($\beta(t)=1$), we extend the range of the hyperparameter, $\beta(t)$, from $0$ to $1$ in our controlVAE model. Given a desired KL-divergence, controlVAE can automatically tune $\beta(t)$ within that range. For this task, we use the same PI control algorithm and hyperparameters as the above language modeling.

%%%%%--language modeling
\item \textbf{Language modeling}: We first apply ControlVAE to solve the KL vanishing problem meanwhile improve the diversity of generated data. As mentioned in Section~\ref{sec:vae-intro}, the VAE models often suffer from KL vanishing in language modeling. The existing methods cannot completely solve the KL vanishing problem or explicitly manipulate the value of KL-divergence. In this paper, we adopt ControlVAE to control KL-divergence to a specified value to avoid KL vanishing using the output KL-divergence. Following PI tuning strategy in Section~\ref{sec:pi_tuning}, we set $K_p$, $K_i$ of the PI algorithm in~\eqref{eq:vae-lang} to $0.01$ and $0.0001$, respectively. In addition, $\beta_{min}$ is set to $0$ and the maximum value of $\beta(t)$ is limited to $1$.

\end{itemize}

%%%--figure for disentanglement
\begin{figure*}[!t]
\centering     %% not \center
\subfigure[Reconstruction loss]{\includegraphics[width=0.32\textwidth]{figures/Sprites_rec_loss.pdf}}
\subfigure[$\beta(t)$]{\includegraphics[width=0.32\textwidth]{figures/Sprites_weight.pdf}}
\subfigure[Disentangled factors]{\includegraphics[width=0.32\textwidth]{figures/Sprites_KL_loss.pdf}}
\caption{(a) (b) shows the comparison of reconstruction error and $\beta(t)$ using 2D Shapes data over $5$ random seeds. ControlVAE (KL=16, 18) and Control-FactorVAE have lower reconstruction errors and variance compared to the other methods. (c) shows an example about the disentangled factors in the latent variable as the total KL-divergence increases from $0.5$ to $18$ for ControlVAE (KL=18). Each curve with positive KL-divergence (except black one) represents one disentangled factor by ControlVAE.}\label{fig:disentangled}
\end{figure*}
